Data-driven finite element method with RVE generated foam data

This paper presents a model-free data-driven strategy for linear and non-linear finite element computations of open-cell foam. Employing sets of material data, the data-driven problem is formulated as the minimization of a distance function subjected to the physical constraints from the kinematics and the balance laws of the mechanical problem. The material data sets of the foam are deduced here from representative microscopic material volumes. These volume elements capture the stochastic characteristics of the open-cell microstructure and the properties of the polyurethane material. Their computation provides the required stress-strain data used in the macroscopic finite element computations without postulating a specific constitutive model. The paper shows how to efficiently derive suitable material data sets for the different (non-)linear and (an-)isotropic material behavior cases. Exemplarily, we compare data-driven finite element computations with linearized and finite deformations and show that a linear kinematic is sufficiently accurate to capture the material's non-linearity up to 50% of straining. The numerical example of a rubber sealing illustrates possible areas of application, the expenditure, and the proposed strategy's versatility.

==> dd2_data_gen_eigen.tex <==
Now, we want to actually conduct data-driven computations. We start with a parametric and comparative study using a one-dimensional rod. Then we show the practical applicability of the method by two examples in a data-driven FEA of a rubber sealing. In the course of the three examples we will increase the complexity of the  macroscopic finite element calculation in the sense that the dimension of the problem is increased. At the same time, however, we increase the requirements on the material in terms of isotropy and linearity in order to reduce the effort. The first example is a one dimensional rod with non-linear material data. The second example is a three dimensional example in the plane strain state with a non-linear isotropic material. And in the last example we compute a full three dimensional example but use linear material data with a small \gruen{anisotropy}.%In both simulations we assume that the material got a complex microstructure, e.g. a foam like structure. Simulations with a representative volume element are used to generate a database of the homogenized material answer.

\subsection{Example 1: 1-D rod example with non-linear data and non-linear geometry}\label{sec:stab}
\gruen{Case A vlt?}
In our first example we conduct a parametric and comparative study on an elongated rod.


\begin{figure}[htb!]
\centering
\includegraphics[width=1\textwidth]{neu/zugstab_ref}
\caption{Reference state of the tapered rod. }\label{fig:Zugstab_ref}
\end{figure}


\subsubsection*{Material data}
Here, the material data is gained from a cylindrical RVE with a foam-like structure. The RVE can be seen in its reference configuration and in a tension state in Fig.\ref{fig:ZylinderRVE}. The cylinder got a height of 300\textmu m and radius of 100\textmu m. The volume ratio is $R=0.15$ and 50 log-normal distributed bubbles are inside the cylinder. For the matrix material we employed two different hyperelastic models. The Neo-Hooke model is used with parameters $C_{10}=3.8461\,$MPa$=\mu/2$ and $D_1=0.12$ MPa$^{-1}=2/K$ which corresponds to a polyurethan solid. The other material model is a Yeoh model with parameters $C_{10}=0.5$MPa$, C_{20}=0, C_{30}=250$MPa$, D_1=0.12$ MPa$^{-1}, D_2=12200$ MPa$^{-1}, D_3=120000$ MPa$^{-1}$ which is used to have a higher grade of non-linearity. The parameter do not belong to a special material. 

\begin{figure}[htb!]
\centering
\includegraphics[width=0.95\textwidth]{neu/zylinder_ref}
\caption{The cylindrical RVE in the reference and a deformed state. }\label{fig:ZylinderRVE}
\end{figure}

Here, we are only interested in one dimensional stretch-stress data. To a given elongation we are only interested in the stress in the direction of the head surface of the cylinder. The lower head surface is fixed and the other is pulled away for different displacements.


\begin{figure}[htb!]
\centering
\includegraphics[width=0.55\textwidth]{neu/data_sets_NH_yeoh}
\caption{Both generated data sets in comparison: The Yeoh model yields a stronger non-linearity. }\label{fig:data_1d}
\end{figure}


\subsection*{Macroscopic level}

%%%%%%%%%%%%%%%%%% Example 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Example 2: Plane 3-D example with non-linear data and linearized geometry}\label{sec:exa2}
Our second example is one that falls into the situation of Case B. The macroscopic structure of a rubber sealing made of a non-linear and isotropic material is computed.
The sealing can be seen in Fig.~\ref{fig:_dichtung}. The width of the bottom side is 35mm, the height is 15mm and the depth 5mm. The thickness of the webs is 1.5mm. The device is typically loaded from atop.

\begin{figure}[htb!]
\centering
\includegraphics[width=0.49\textwidth]{neu/dichtung_2}
\includegraphics[width=0.49\textwidth]{neu/dichtung_1}
\caption{The rubber gasket component.}\label{fig:_dichtung}
\end{figure}





\subsection*{Material data}
In the first example we needed a rather small data set due to the dimension of the problem considered in the macroscopic finite element simulation. In this example we have a three dimensional example, however, we reduce the numerical costs by assuming a plane strain state. A plane RVE is used therefore. The RVE can be seen in Fig. \ref{fig:rve_ebene_simul} in its reference configuration as well as in one of the 2601 deformations it was subjected to. The matrix material is the same Neo-Hooke material as in example 1 which corresponds to a polyurethan material, e.g. $C_{10}=3.8461\,$MPa and $D_1=0.12$ MPa$^{-1}$. The principal strain components $\epsilon_1$ and $\epsilon_2$ were varied by 51 values between $\pm 0.2$ leading to 2601 simulations with the RVE. The 2601 data points with different values in the principal directions are then rotated by 72 different angles. Due to the reduction to the plane strain state we only need to do the rotations around the $z$-axis. This leads to a data set of $2601\cdot 73=189873$ data tuples which are put in the data-driven simulation as initial set for the multi-level simulation. A linear approximation of the homogenized material behavior yields a Young's modulus around 13 MPa.
\begin{figure}[htb!]
\centering
\includegraphics[width=1\textwidth]{neu/rve_ebene_combined}
\caption{The plane RVE in its reference state and a deformed state. The displacement in $x$-direction is 0.0728 mm and in $y$-direction 0.05040.}\label{fig:rve_ebene_simul}
\end{figure}

\subsection*{Macroscopic finite element simulation}
\gruen{Datenpunkte F,P? Rechnung eps sigma}
The rubber sealing and its boundary conditions can be seen on the left-hand side in Fig.~\ref{fig:examp2_bc}. Furthermore, the component is fixed in the $z$-direction. For the surface load $p$ three different values are used, namely $p\in\{0.003,0.01,0.03\}$ MPa.
\begin{figure}[htb!]
\centering
\includegraphics[width=0.48\textwidth]{neu/Gummi_mesh_BC_AUTO}
\includegraphics[width=0.48\textwidth]{neu/lastverschiebung_paper_exa2}
\caption{Mesh and boundary conditions of rubber sealing.}\label{fig:examp2_bc}
\end{figure}
For comparison purposes, linear and non-linear FEM calculations based on classical material models were also performed. On the right-hand side of Fig.~\ref{fig:examp2_bc} a load-displacement curve is shown for the two classic finite element solutions as well as for the data-driven solution. The displacement was recorded in the middle of the top nodes where the biggest displacement occurs. It can be seen that the data-driven solution is in coincidence with the other classic computations in the linear load regime. However, in the non-linear regime the data-driven solution does not reproduce the non-linear material behavior of the data set which is put in. Neither is the linear solution reproduced. From our point of view this is the result of the linearized kinematics together with the non-linear material set. The data-driven computations were run with 3 level of refined data sets. In Table \ref{table:MLex2} the size of the input data set is shown as well as the number of data tuples which are actually assigned to a material point from the simulation with the highest load.
\begin{table}
\centering
\ra{1.2}
\begin{tabular}{crc}\toprule
Level $l$  & data tuples in $\mathcal{D}_l$& data tuples in $\mathcal{S}_l$   \\ \hline
0 & 189.873 & 2.972    \\

1 & 80.244 & 3.197  \\

2 & 86.319 & 5.201  \\\hline
\bottomrule
\end{tabular}
\caption{Sizes of the input data and the number of data tuples describing the material of the multi level computation.  }
\label{table:MLex2}
\end{table}


In Fig.~\ref{fig:examp2_stress} the stress component $\sigma_x$ is displayed for the highest surface load. While the overall stress distribution looks roughly the same the values are rather different.




\begin{figure}[htb!]
\centering
\includegraphics[width=0.68\textwidth]{neu/ML2_DD_sig11_paper_exa2}
\includegraphics[width=0.68\textwidth]{neu/CLAS_sig11_paper_exa2}
\caption{Stress component $\sigma_{x}$ for the data-driven (left) and the classic solution for a surface load $p=0.03$ MPa.}\label{fig:examp2_stress}
\end{figure}




%%%%%%%%%%%%%%%%%% Example 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Example 3/Case C: 3-D example with linear Data and linearized kinematics }\label{sec:exa3}
In the last example we compute the rubber sealing again. But this time in a full three dimensional deformation state with a different loading scenario. While in the two previous examples the RVEs are rather of exemplary nature, in this example a model is chosen which has the claim to reproduce the properties of a polyurethane foam exactly. Since foam is typically used in the linear load range and since the underlying RVE is also very complex to calculate numerically, this example falls into the case C.






\subsubsection*{Material data}
 The RVE which is presented in section \ref{sec:rve} is used now. For the sake of completeness we repeat once again the parameters of the RVE. The size of the RVE is $1000\times 1000\times 1000\,$\textmu m and got a relative density of $R=0.15$ . The  RVE has {100 log-normally distributed  pores} with a coefficient of variation $CV=0.5$  and it is meshed with 708\,372 elements tetragonal solid elements. In case C we need to compute 6 different computation. In case C we need 6 simulations to cover the linear load range, one of them is shown in \ref{fig:rve_wurfel_simul}. The right surface of the cube is pulled away from the rest of the body. You can clearly see that the stress is highest in the webs that are orientated in this direction. The six evaluated data tuples can be seen in the appendix. Due to the random sphere packing in the generation process there are small deviations of the different directions.  \gruen{Können wir das schreiben? Machen wir dadurch die Bezeichnung RVE kaputt? Ansonsten sind wir eigentlich in Fall D wenn wir sagen es ist isotrop.}



\begin{figure}[htb!]
\centering
\includegraphics[width=1\textwidth]{neu/rve_lukas_combined}
\caption{The unloaded and loaded RVE of the PUR RVE for a displacement in the $x$-direction.}\label{fig:rve_wurfel_simul}
\end{figure}

\subsection*{Macroscopic finite element simulation}
Lastly, we compute a full three dimensional example. The boundary conditions do not change significantly in contrast to example 2. The component is not fixed in the $z$-direction anymore but still fixed at the bottom side. The surface load from atop still exists now indicated as $p_1$ as we add two additional surface loads $p_2$ pointing into the $z$-direction. One pushes the rubber sealing in the third direction while on the other  the sealing is pulled. As this example is intended to be in the linear load regime we lower the surface load from above to $p_1=-7.5\cdot 10^{-3}$ MPa. The surface load $p_2$ is of magnitude $p_2=2.5\cdot 10^{-2}$ MPa.

\begin{figure}[htb!]
\centering 
\includegraphics[width=0.48\textwidth]{neu/Gummi_mesh_BC3}
\includegraphics[width=0.48\textwidth]{neu/exa3_BC2}
\caption{Mesh and boundary conditions of the rubber sealing in example 3. An additional surface load in $z$-direction is added (red). On the right-hand side the elements effected by $p_1$ are in darker green.}\label{fig:examp3_bc}
\end{figure}


In Fig.\ref{fig:examp3_13} the shear stress is plotted of a reference and the data-driven solution. The displacement is magnified by 5 such that the torsion of the component can be seen. The data-driven solution is got the typical patchy contours which indicates that still some data points are missing.
\begin{figure}[htb!]
\centering 
\includegraphics[width=0.98\textwidth]{neu/combined_exa3_REF_S13_gros}
\caption{Shear stress $\tau_{13}$ in the rubber sealing. The data-driven solution is still a little bit patchy indicating a refinement can still yield better results.}\label{fig:examp3_13}
\end{figure}



